Higher tensor categories and their extensions: notes from the Scottish Talbot On Algebra and Topology

These lecture notes are the product of a week-long learning workshop on the work of Johnson-Freyd and Reutter on the problem of the existence of minimal nondegenerate extensions of braided fusion categories (arXiv:2105.15167). They recount the mathematical arguments of the original paper from an expository angle, with background material covering the algebra and homotopy theory required to understand the statement and follow the proof. The notes are aimed at newcomers to the field of (braided) fusion 1- and 2-categories.

==> talks/3.1/Preamble.tex <==
\usepackage{vmargin}
\setmarginsrb{28mm}{25mm}{28mm}{25mm}{0pt}{0mm}{0pt}{0mm}
\setlength{\footskip}{20pt}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{pgfplots} 
\usepackage{graphicx}
\usepackage{wrapfig}
\graphicspath{ {./images/} }
\usepackage[utf8x]{inputenc}
\usepackage{tikz-cd}
\usepackage{tikz}
\usetikzlibrary{arrows,arrows.meta,%
	decorations.markings,decorations.pathreplacing,%
	decorations.pathmorphing,calc}
\usepackage{bbm}
\usepackage{subcaption}
\usepackage[boxruled]{algorithm2e}
\usepackage{mathtools}
\usepackage{lipsum}
\usepackage[title,titletoc]{appendix}
\usepackage{booktabs}
\usepackage{here}
\usepackage[]{hyperref}
\usepackage{natbib,enumerate}
\usepackage{euscript}
\usepackage{unicode-math}

\usepackage[nottoc]{tocbibind} % References in ToC
\bibliographystyle{plain}	% a modified version of alpha.bst by zzh

%some weird packages
\usepackage{halloweenmath}
\usepackage{txfonts}
\usepackage{knitting}

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\renewcommand{\phi}{\varphi}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{#1}{=}}}
\newcommand{\leqtext}[1]{\ensuremath{\stackrel{#1}{\leq}}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{example}{Example}[section]
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\epl}{\varepsilon}
\newcommand\Cb			{\mathbb{C}}
\newcommand\Fb          {\mathbb{F}}
\newcommand\Hb			{\mathbb{H}}
\newcommand\Nb			{\mathbb{N}}
\newcommand\Pb			{\mathbb{P}}
\newcommand\Qb			{\mathbb{Q}}
\newcommand\Rb			{\mathbb{R}}
\newcommand\Sb          {\mathbb{S}}
\newcommand\Zb			{\mathbb{Z}}
\newcommand\Kb          {\mathbb{K}}
\newcommand\kb			{\mathbb{k}}

\newcommand\CA			{\EuScript{A}}
\newcommand\CB			{\EuScript{B}}
\newcommand\CC			{\EuScript{C}}
\newcommand\CD			{\EuScript{D}}
\newcommand\CE			{\EuScript{E}}
\newcommand\CF			{\EuScript{F}}
\newcommand\CG			{\EuScript{G}}
\newcommand\CH			{\EuScript{H}}
\newcommand\CI			{\EuScript{I}}
\newcommand\CJ			{\EuScript{J}}
\newcommand\CK			{\EuScript{K}}
\newcommand\CL			{\EuScript{L}}
\newcommand\CM			{\EuScript{M}}
\newcommand\CN			{\EuScript{N}}
\newcommand\CO			{\EuScript{O}}
\newcommand\CP			{\EuScript{P}}
\newcommand\CQ			{\EuScript{Q}}
\newcommand\CR			{\EuScript{R}}
\newcommand\CS			{\EuScript{S}}
\newcommand\CT			{\EuScript{T}}
\newcommand\CU			{\EuScript{U}}
\newcommand\CV			{\EuScript{V}}
\newcommand\CW			{\EuScript{W}}
\newcommand\CX			{\EuScript{X}}
\newcommand\CY			{\EuScript{Y}}
\newcommand\CZ			{\EuScript{Z}}

\newcommand\Ac			{\mathcal{A}}
\newcommand\Bc			{\mathcal{B}}
\newcommand\Cc			{\mathcal{C}}
\newcommand\Dc			{\mathcal{D}}
\newcommand\Ec			{\mathcal{E}}
\newcommand\Fc			{\mathcal{F}}
\newcommand\Gc			{\mathcal{G}}
\newcommand\Hc			{\mathcal{H}}
\newcommand\Ic			{\mathcal{I}}
\newcommand\Jc			{\mathcal{J}}
\newcommand\Kc			{\mathcal{K}}
\newcommand\Lc			{\mathcal{L}}
\newcommand\Mc			{\mathcal{M}}
\newcommand\Nc			{\mathcal{N}}
\newcommand\Oc			{\mathcal{O}}
\newcommand\Pc			{\mathcal{P}}
\newcommand\Rc			{\mathcal{R}}
\newcommand\Qc			{\mathcal{Q}}
\newcommand\Sc			{\mathcal{S}}
\newcommand\Tc			{\mathcal{T}}
\newcommand\Uc			{\mathcal{U}}
\newcommand\Vc			{\mathcal{V}}
\newcommand\Wc			{\mathcal{W}}
\newcommand\Xc			{\mathcal{X}}
\newcommand\Yc			{\mathcal{Y}}
\newcommand\Zc			{\mathcal{Z}}


\newcommand{\FA}			{\mathfrak{A}}
\newcommand{\FB}			{\mathfrak{B}}
\newcommand{\FC}			{\mathfrak{C}}
\newcommand{\FD}			{\mathfrak{D}}
\newcommand{\FE}			{\mathfrak{E}}
\newcommand{\FF}			{\mathfrak{F}}
\newcommand{\FG}			{\mathfrak{G}}
\newcommand{\FH}			{\mathfrak{H}}
\newcommand{\FI}			{\mathfrak{I}}
\newcommand{\FJ}			{\mathfrak{J}}
\newcommand{\FK}			{\mathfrak{K}}
\newcommand{\FL}			{\mathfrak{L}}
\newcommand{\FM}			{\mathfrak{M}}
\newcommand{\FN}			{\mathfrak{N}}
\newcommand{\FO}			{\mathfrak{O}}
\newcommand{\FP}			{\mathfrak{P}}
\newcommand{\FQ}			{\mathfrak{Q}}
\newcommand{\FR}			{\mathfrak{R}}
\newcommand{\FS}			{\mathfrak{S}}
\newcommand{\FT}			{\mathfrak{T}}
\newcommand{\FU}			{\mathfrak{U}}
\newcommand{\FV}			{\mathfrak{V}}
\newcommand{\FW}			{\mathfrak{W}}
\newcommand{\FX}			{\mathfrak{X}}
\newcommand{\FY}			{\mathfrak{Y}}
\newcommand{\FZ}			{\text{\usefont{U}{euf}{m}{n}Z}}
\newcommand{\Fp}			{\mathfrak{p}}
\newcommand{\Fg}            {\mathfrak{g}}
\newcommand{\Fh}            {\mathfrak{h}}
\newcommand{\Fn}            {\mathfrak{n}}


\newcommand\BA			{\mathbf{A}}
\newcommand\BB			{\mathbf{B}}
\newcommand\BC			{\mathbf{C}}
\newcommand\BD			{\mathbf{D}}
\newcommand\BE			{\mathbf{E}}
\newcommand\BF			{\mathbf{F}}
\newcommand\BG			{\mathbf{G}}
\newcommand\BH			{\mathbf{H}}
\newcommand\BI			{\mathbf{I}}
\newcommand\BJ			{\mathbf{J}}
\newcommand\BK			{\mathbf{K}}
\newcommand\BL			{\mathbf{L}}
\newcommand\BM			{\mathbf{M}}
\newcommand\BN			{\mathbf{N}}
\newcommand\BO			{\mathbf{O}}
\newcommand\BP			{\mathbf{P}}
\newcommand\BR			{\mathbf{R}}
\newcommand\BQ			{\mathbf{Q}}
\newcommand\BS			{\mathbf{S}}
\newcommand\BT			{\mathbf{T}}
\newcommand\BU			{\mathbf{U}}
\newcommand\BV			{\mathbf{V}}
\newcommand\BW			{\mathbf{W}}
\newcommand\BX			{\mathbf{X}}
\newcommand\BY			{\mathbf{Y}}
\newcommand\BZ			{\mathbf{Z}}
\newcommand\BGL         {\mathbf{GL}}
\newcommand\BSL         {\mathbf{SL}}
\newcommand\BSO         {\mathbf{SO}}
\newcommand\BSp         {\mathbf{Sp}}

\newcommand\SA			{\mathsf{A}}
\newcommand\SB			{\mathsf{B}}
\newcommand\SC			{\mathsf{C}}
\newcommand\SD			{\mathsf{D}}
\newcommand\SE			{\mathsf{E}}
\newcommand\SF			{\mathsf{F}}
\newcommand\SG			{\mathsf{G}}
\newcommand\SH			{\mathsf{H}}
\newcommand\SI			{\mathsf{I}}
\newcommand\SJ			{\mathsf{J}}
\newcommand\SK			{\mathsf{K}}
\newcommand\SL			{\mathsf{L}}
\newcommand\SM			{\mathsf{M}}
\newcommand\SN			{\mathsf{N}}
\newcommand\SO			{\mathsf{O}}
\newcommand\SP			{\mathsf{P}}
\newcommand\SQ			{\mathsf{Q}}
\newcommand\SR			{\mathsf{R}}
%\newcommand\SS			{\mathsf{S}}
\newcommand\ST			{\mathsf{T}}
\newcommand\SV			{\mathsf{V}}
\newcommand\SW			{\mathsf{W}}
\newcommand\SX			{\mathsf{X}}
\newcommand\SY			{\mathsf{Y}}
\newcommand\SZ			{\mathsf{Z}}

%\newcommand{\ising}{\mathbf{Is}}
%\newcommand{\toric}{\mathbf{Toric}}
\newcommand{\Ising}{\mathrm{Is}}
\newcommand{\Toric}{\mathrm{Toric}}

\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\coim}{coim}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Pro}{Pro}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\holim}{holim}
\DeclareMathOperator{\hocolim}{hocolim}
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\fib}{fib}
\DeclareMathOperator{\cofib}{cofib}
\DeclareMathOperator{\coev}{coev}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\Kom}{Kom}

\DeclareMathOperator{\fpdim}{FPdim}
\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\ob}{ob}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\nord}{nord}
\DeclareMathOperator{\orm}{or}
\DeclareMathOperator{\fr}{fr}
\DeclareMathOperator{\br}{br}

\DeclareMathOperator{\Presh}{Presh}

%\DeclareMathOperator{\Set}{\EuScript{S}\mathrm{et}}
\DeclareMathOperator{\nat}{Nat}
\DeclareMathOperator{\fun}{Fun}
\DeclareMathOperator{\Fun}{\EuScript{F}\mathrm{un}}
\DeclareMathOperator{\BiFun}{BiFun}
\DeclareMathOperator{\Map}{Map}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\CHom}{CHom}
\DeclareMathOperator{\Idem}{Idem}
\DeclareMathOperator{\Ret}{Ret}
\DeclareMathOperator{\Mul}{Mul}
\DeclareMathOperator{\Fin}{Fin}
\DeclareMathOperator{\Vect}{Vect}
\DeclareMathOperator{\Ch}{Ch}
\DeclareMathOperator{\Alg}{Alg}
\DeclareMathOperator{\CAlg}{CAlg}
\DeclareMathOperator{\coAlg}{coAlg}
\DeclareMathOperator{\coCAlg}{coCAlg}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Free}{Free}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\Mod}{Mod}
\DeclareMathOperator{\BrMod}{BrMod}
\DeclareMathOperator{\LMod}{LMod}
\DeclareMathOperator{\RMod}{RMod}
\DeclareMathOperator{\BMod}{BMod}
\DeclareMathOperator{\sHBA}{sHBA}
\DeclareMathOperator{\Mon}{Mon}
\DeclareMathOperator{\Step}{Step}
\DeclareMathOperator{\Barr}{Bar}
\DeclareMathOperator{\Cobar}{Cobar}
\DeclareMathOperator{\LinFun}{LinFun}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\PSp}{PSp}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Exc}{Exc}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Emb}{Emb}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Homeo}{Homeo}
\DeclareMathOperator{\CRing}{CRing}
\DeclareMathOperator{\Aff}{Aff}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Sch}{Sch}
\DeclareMathOperator{\Str}{Str}
\DeclareMathOperator{\RingTop}{RingTop}
\DeclareMathOperator{\SpSch}{SpSch}
\DeclareMathOperator{\Stk}{Stk}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\QCoh}{QCoh}
\DeclareMathOperator{\map}{Map}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\Conn}{Conn}
\DeclareMathOperator{\LocSys}{LocSys}
\DeclareMathOperator{\Disk}{Disk}
\DeclareMathOperator{\Mfld}{Mfld}
\newcommand{\CDisk}			{\EuScript{D}\mathrm{isk}}
\newcommand{\CMfld}			{\EuScript{M}\mathrm{fld}}
\newcommand{\bDisk}         {\mathbb{D}\mathrm{isk}}
\newcommand{\Surf}          {\mathbb{S}\mathrm{urf}}

\newcommand{\Grp}			{\mathrm{Grp}}
\newcommand{\Var}			{\mathrm{Var}}
\newcommand{\Open}			{\mathrm{Open}}
\newcommand{\op}			{\mathrm{op}}
\newcommand{\rev}			{\mathrm{rev}}
\newcommand{\flp}			{\mathrm{flp}}
\newcommand{\one}			{\mathbb{1}}

\newcommand\bh{\mathbf{H}}
\newcommand\en{\mathrm{en}}
\newcommand\forget  {\mathbf{f}}
\newcommand\cl  {\mathrm{bulk}}

\newcommand\Cat			{\EuScript{C}\mathrm{at}}
\newcommand\cat			{\mathrm{Cat}}
\newcommand\Set			{\EuScript{S}\mathrm{et}}
\newcommand\set			{\mathrm{Set}}
\newcommand\sSet			{\mathbf{sSet}}
\newcommand\nvect			{n\mathrm{Vec}}
\newcommand\vect			{\mathrm{Vec}}
\newcommand\svect			{\mathrm{sVec}}
\newcommand\hilb			{\mathrm{Hilb}}
\newcommand\Rep			{\EuScript{R}\mathrm{ep}}
\newcommand\rep			{\mathrm{Rep}}
%\newcommand\Mat			{\EuScript{M}\mathrm{at}}
%\newcommand\alg			{\EuScript{A}\mathrm{lg}}
%\newcommand\cTop			{\mathrm{Top}}
%\newcommand\Topo			{\EuScript{T}\mathrm{op}}
%\newcommand\grp			{\EuScript{G}\mathrm{rp}}
%\newcommand\ring			{\EuScript{R}\mathrm{ing}}
%\newcommand\abel			{\EuScript{A}\mathrm{bel}}
%\newcommand\cring			{\EuScript{C}\mathrm{ring}}
%\newcommand\Ab			{\mathrm{Ab}}

\newcommand\nao			{\mbox{$n$+1}}
\newcommand\nmo			{\mbox{$n$-1}}
\newcommand\Pic			{\mathrm{Pic}}
\newcommand\Irr			{\mathrm{Irr}}
